Enabling Team of Teams: A Trust Inference and Propagation (TIP) Model in Multi-Human Multi-Robot Teams

Trust has been identified as a central factor for effective human-robot teaming. Existing literature on trust modeling predominantly focuses on dyadic human-autonomy teams where one human agent interacts with one robot. There is little, if not no, research on trust modeling in teams consisting of multiple human agents and multiple robotic agents. To fill this research gap, we present the trust inference and propagation (TIP) model for trust modeling in multi-human multi-robot teams. In a multi-human multi-robot team, we postulate that there exist two types of experiences that a human agent has with a robot: direct and indirect experiences. The TIP model presents a novel mathematical framework that explicitly accounts for both types of experiences. To evaluate the model, we conducted a human-subject experiment with 15 pairs of participants (${N=30}$). Each pair performed a search and detection task with two drones. Results show that our TIP model successfully captured the underlying trust dynamics and significantly outperformed a baseline model. To the best of our knowledge, the TIP model is the first mathematical framework for computational trust modeling in multi-human multi-robot teams.

==> backup/old_text_backup.tex <==
%%%%%%%%% old casy-by-case theorems %%%%%%%%%%%%%%%%
\noindent\textbf{Case 1}: $m=0$ and $n >0$. In this case, $y$ only works with $A$ directly and $x$ only update his or her trust on $A$ indirectly through $y$. Theorem \ref{thm1} shows $y$'s trust on $A$ converges to a constant.

\begin{theorem}
\label{thm1}
When $m=0$ and $n >0$, $y$'s trust $t_{A}^{y}( k)$ on $A$ converges to $\frac{s_{A}^{y} r}{f_{A}^{y}\overline{r} +s_{A}^{y} r}$ in probability, i.e., for any $\epsilon  >0$,
\begin{equation*}
\lim _{k\rightarrow \infty } P\left(\left| t_{A}^{y}( k) -\frac{s_{A}^{y} r}{f_{A}^{y}\overline{r} +s_{A}^{y} r}\right|  >\epsilon \right) = 0.
\end{equation*}
\end{theorem}


\begin{theorem}
\label{thm2}
When $m=0$ and $n >0$, the difference between $t_{A}^{x}( k)$ and $t_{A}^{y}( k)$ converge to 0 in probability, i.e., for any $\epsilon  >0$,
\begin{equation*}
\lim _{k\rightarrow \infty } P\left(\left| t_{A}^{x}( k) -t_{A}^{y}( k)\right|  >\epsilon \right) = 0.
\end{equation*}
\end{theorem}

\noindent\textbf{Case 2}: $m >0$ and $n >0$. In this case, each agent can work with the robot both directly and indirectly. We have the following main result:
\begin{theorem}
\label{thm3}
When $m >0$ and $n >0$, $t_{A}^{x}( k)$ and $t_{A}^{y}( k)$ converge in probability respectively, i.e., there exists $t_{A}^{x}$ and $t_{A}^{y}$ such that, for any $\epsilon  >0$,
\begin{equation*}
\begin{aligned}
 &  & \lim _{k\rightarrow \infty } P\left(\left| t_{A}^{x}( k) -t_{A}^{x}\right|  >\epsilon \right) =0,\ \\
\text{ and } &  & \lim _{k\rightarrow \infty } P\left(\left| t_{A}^{y}( k) -t_{A}^{y}\right|  >\epsilon \right) =0.
\end{aligned}
\end{equation*}
\end{theorem}


\begin{theorem}
\label{thm4}
The equilibria $t_{A}^{x}$ and $t_{A}^{y}$ in Theorem \ref{thm3} satisfy
\begin{gather}\label{eq:thm4_1}
\text{ \ \ \ \ } \ \ \begin{aligned}
\left( 1-t_{A}^{x}\right) /t_{A}^{x} & =\left[\hat{F}_{A}^{x}\left( t_{A}^{x} -t_{A}^{y}\right) +F_{A}^{x}\right] /S_{A}^{x}
\end{aligned} \\
\text{and \ }\begin{aligned} \label{eq:thm4_2}
\left( 1-t_{A}^{y}\right) /t_{A}^{y} & = F_{A}^{y} /\left[\hat{S}_{A}^{y}\left( t_{A}^{x} -t_{A}^{y}\right) +S_{A}^{y}\right],
\end{aligned}
\end{gather}
if $S_{A}^{x} /F_{A}^{x} -S_{A}^{y} /F_{A}^{y} \geqslant 0$; otherwise, they satisfy
\begin{gather}
\text{ \ \ \ \ } \ \ \begin{aligned} \label{eq:thm4_3}
\left( 1-t_{A}^{x}\right) /t_{A}^{x} & =F_{A}^{x} /\left[\hat{S}_{A}^{x}\left( t^{y} -t^{x}\right) +S_{A}^{x}\right]
\end{aligned} \\
\text{and \ }\begin{aligned} \label{eq:thm4_4}
\left( 1-t_{A}^{y}\right) /t_{A}^{y} & =\left[\hat{F}_{A}^{y}\left( t^{y} -t^{x}\right) +F_{A}^{y}\right] /S_{A}^{y},
\end{aligned}
\end{gather}
where $\hat{S}_{A}^{x} =nt_{y}^{x}\hat{s}_{A}^{x}$, $\hat{F}_{A}^{x} =nt_{y}^{x}\hat{f}_{A}^{x}$, $S_{A}^{x} =ms_{A}^{x} r$, $F_{A}^{x} =mf_{A}^{x}\overline{r}$, $\hat{S}_{A}^{y} =mt_{x}^{y}\hat{s}_{A}^{y}$, $\hat{F}_{A}^{y} =mt_{x}^{y}\hat{f}_{A}^{y}$, $S_{A}^{y} =ns_{A}^{y} r$, and $F_{A}^{y} =nf_{A}^{y}\overline{r}$.

\end{theorem}



%%%%%%%%%%%%%% old proofs %%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem \ref{thm:both_converge}}
As $m=0$ and $n >0$, $y$ only gains experience towards robot $A$ through direct interaction. Therefore, by Eq.~\eqref{eq:direct_update},
\begin{equation*}
\begin{aligned}
 & \lim _{k\rightarrow \infty }\frac{\alpha _{A}^{y}( k)}{\alpha _{A}^{y}( k) +\beta _{A}^{y}( k)}\\
= & \lim _{k\rightarrow \infty }\frac{\alpha _{A}^{y}( 0) +kns_{A}^{y} r}{\alpha _{A}^{y}( 0) +\beta _{A}^{y}( 0) +knf_{A}^{y}\overline{r} +kns_{A}^{y} r}\\
= & \lim _{k\rightarrow \infty }\frac{kns_{A}^{y} r}{knf_{A}^{y}\overline{r} +kns_{A}^{y} r} =\frac{s_{A}^{y} r}{f_{A}^{y}\overline{r} +s_{A}^{y} r} .
\end{aligned}
\end{equation*}



\subsection{Proof of Theorem \ref{thm:equilibria}}
Suppose the claim is not true. Then there exist $\epsilon ,\ \delta  >0$ such that there is infinite many $i$ such that $P\left(\left| t_{A}^{x}( i) -t_{A}^{y}( i)\right|  >\epsilon \right)  >\delta $. Let $\{i_{k}\}_{k}$ be a sequence of such $i$s. Let $q=\min\left\{t_{y}^{x}\hat{f}_{A}^{x} ,\ t_{y}^{x}\hat{s}_{A}^{x}\right\}$. By Eq.~\eqref{eq:indirect_update}, 
\begin{equation}\label{eq:bound1}
\begin{aligned}
 & \alpha _{A}^{x} (k)+\beta _{A}^{x} (k)-\alpha _{A}^{x} (k-1)-\beta _{A}^{x} (k-1)\\
\geqslant  & q\left| t_{A}^{x} (k-1)-t_{A}^{y} (k)\right| .
\end{aligned}
\end{equation}
Define i.i.d. random variables $d_{k}$ by $P( d_{k} =\epsilon ) =\delta $ and $P( d_{k} =0) =1-\delta $, for $k=1,2,\dotsc $. Let $\gamma $ be an arbitrary positive number. Then,
\begin{equation*}
\begin{aligned}
 & \lim _{k\rightarrow \infty } P\left( \alpha _{A}^{x} (i_{k} )+\beta _{A}^{x} (i_{k} ) >\gamma \right)\\
\geqslant  & \lim _{k\rightarrow \infty } P\left( \alpha _{A}^{x} (i_{k} )+\beta _{A}^{x} (i_{k} )-\alpha _{A}^{x} (0)-\beta _{A}^{x} (0) >\gamma \right)\\
\geqslant  & \lim _{k\rightarrow \infty } P\left(\sum\nolimits _{j=1}^{i_{k}} q\left| t_{A}^{x} (j-1)-t_{A}^{y} (j)\right|  >\gamma \right)\\
\geqslant  & \lim _{k\rightarrow \infty } P\left(\sum\nolimits _{j=1}^{k} q\left| t_{A}^{x} (i_{k} -1)-t_{A}^{y} (i_{k} )\right|  >\gamma \right)\\
\geqslant  & \lim _{k\rightarrow \infty } P\left(\sum\nolimits _{j=1}^{k} qd_{j}  >\gamma \right)\\
= & \lim _{k\rightarrow \infty } P\left(\frac{\sum\nolimits _{j=1}^{k} d_{j}}{k}  >\frac{\gamma }{qk}\right) =1,
\end{aligned}
\end{equation*}
where the second inequality is true because of Eq.~\eqref{eq:bound1} and the last line is true because of the law of large numbers. Since $\gamma $ is an arbitrary number, the above equation shows $\alpha _{A}^{x} (k)+\beta _{A}^{x} (k)\rightarrow \infty $ as $k\rightarrow \infty $. Further more, when $\alpha _{A}^{x} (k)+\beta _{A}^{x} (k)\rightarrow \infty $, \ $\left| t_{A}^{x}( k) -\E\left[ t_{A}^{x}( k)\right]\right| $ converges to zero. For $y$, as
\begin{equation}
\begin{aligned}
 & \lim _{k\rightarrow \infty }\left( \alpha _{A}^{y} (k)+\beta _{A}^{y} (k)\right)\\
\geqslant  & \lim _{k\rightarrow \infty }\left(\sum _{j=1}^{k} s_{A}^{y} p_{A}( j) +f_{A}^{y}\overline{p}_{A}( j)\right) =\infty ,
\end{aligned}
\end{equation}
$\left| t_{A}^{y}( k) -\E\left[ t_{A}^{y}( k)\right]\right| $ also converges to zero. By theorem 1, $\lim\limits _{k\rightarrow \infty } \E\left[ t_{A}^{y}( k)\right] =s_{A}^{y} r\left[ s_{A}^{y} r+f_{A}^{y}( 1-r)\right]^{-1}$, which is a constant. A further examination on Eq.~\eqref{eq:indirect_update} indicates $t_{A}^{y} (k)-t_{A}^{x} (k)$ also converges to zero, contradicting our assumption.

\subsection{Proof of Theorem \ref{thm3}}
A formal proof is long as it needs multiple $\epsilon -\delta $ arguments. We provide a proof sketch instead.

First, we show, when $k\rightarrow \infty $, $\alpha _{A}^{x} (k )$, $\beta _{A}^{x} (k)$, $\alpha _{A}^{y} (k )$, and $\beta _{A}^{y} (k)$ all tend to infinity as both $x$ and $y$ will have an infinite number of direct interactions with $A$. As a result, $t_{A}^{x}( k) -\E\left[ t_{A}^{x}( k)\right]$ and $t_{A}^{y}( k) -\E\left[ t_{A}^{y}( k)\right]$ converge to zero.

Second, we show the trust difference between $x$ and $y$ converges to some constant. \ Define random variable $\Delta t(k) :=t_{A}^{x}( k) -t_{A}^{y}(k)$. We can show $\Delta t(k)$ is Cauchy in probability and thus $\Delta t(k)$ converges to some random variable $\Delta t$. As 
\begin{equation*}
\begin{aligned}
 & \Delta t(k) -\E[ \Delta t( k)]\\
= & t_{A}^{x}( k) -\E\left[ t_{A}^{x}(k)\right] -t_{A}^{y}(k) -\E\left[ t_{A}^{y}(k)\right] ,
\end{aligned}
\end{equation*}
where the right hand side converges to zero, $\Delta t(k)$ also converges to zero, i.e, $\Delta t\equiv 0$.

Finally, by Eq.~\eqref{eq:direct_update} update and Eq.~\eqref{eq:indirect_update}, both indirect and direct experience gains converge to some constants. Therefore, the ratio
\begin{equation*}
\frac{\ \alpha _{A}^{x} (k)}{\alpha _{A}^{x} (k)+\beta _{A}^{x} (k)} \ \text{and} \ \ \frac{\alpha _{A}^{x} (k)}{\alpha _{A}^{x} (k)+\beta _{A}^{x} (k)}
\end{equation*}
converge respectively.

\subsection{Proof of Theorem \ref{thm4}}
The subsequences $\left\{t_{A}^{x}( kl)\right\}_{k}$ and $\left\{t_{A}^{y}( kl)\right\}_{k}$ have the same equilibria $t_{A}^{x}$ and $t_{A}^{y}$, where $l=m+n$. If $S_{A}^{x} /F_{A}^{x} -S_{A}^{y} /F_{A}^{y} \geqslant 0$, it can be shown that
\begin{equation*}
\lim\limits _{k\rightarrow \infty } P\left( t^{x}( kl) -t^{y}( kl) \geqslant 0\right) =1.
\end{equation*}
As a result, 
\begin{equation}\label{eq:pos_simplify}
\left[ t_{A}^{y} -t_{A}^{x}\right]^{+} =0\ \text{ and } \ \left[ t_{A}^{x} -t_{A}^{y}\right]^{+} =t^{x} -t^{y} .
\end{equation}
Taking $k$ to $\infty $, by Eq.~\eqref{eq:direct_update}, Eq.~\eqref{eq:indirect_update}, and Eq.~\eqref{eq:pos_simplify}, we have 
\begin{equation}\label{eq:exp_diff_long_run}
\begin{aligned}
\alpha _{A}^{x} (kl+l)-\alpha _{A}^{x} (kl) & =S_{A}^{x}\\
\beta _{A}^{x} (kl+l)-\beta _{A}^{x} (kl) & =\hat{F}_{A}^{x}\left( t_{A}^{x} -t_{A}^{y}\right) +F_{A}^{x}
\end{aligned} ,
\end{equation}
which implies the trust gains are constant every other $l$ interactions. As $\left\{t_{A}^{x}( kl)\right\}_{k}$ converges to $t_{A}^{x}$, by Eq.~\eqref{eq:trust_def},
\begin{equation}\label{eq:txA_limit}
t_{A}^{x} =\lim _{k\rightarrow \infty }\frac{\alpha _{A}^{x} (kl)}{\beta _{A}^{x} (kl)+\alpha _{A}^{x} (kl)} .
\end{equation}
 By Eq.~\eqref{eq:exp_diff_long_run} and Eq.~\eqref{eq:txA_limit}, we can derive Eq.~\eqref{eq:thm4_1}. Eq.~\eqref{eq:thm4_2} can be obtained similarly.

The proof for the case when $S_{A}^{x} /F_{A}^{x} -S_{A}^{y} /F_{A}^{y} < 0$ is similar.

\subsection{Compute $t^x_A$ and $t^y_A$}
We consider the case for Eq.~\eqref{eq:thm4_1} and Eq.~\eqref{eq:thm4_2}. Solving $t^x_A$ in Eq.~\eqref{eq:thm4_1} and substituting the solution to Eq.~\eqref{eq:thm4_2} result in a cubic equation of $t^y_A$. An exact solution can be derived from this cubic equation on $[0,1]^2$ but the process can be tedious. A more practical method is to exploit the Newton's method to approximate $t^x_A$ and $t^y_A$. For example, letting $z=1-y$, Eq.~\eqref{eq:thm4_1} and Eq.~\eqref{eq:thm4_2} give
\begin{equation}
\begin{aligned}
 & \hat{F}_{A}^{x} x^{2} +\hat{F}_{A}^{x} zx+\left( F_{A}^{x} +S_{A}^{x} -\hat{F}_{A}^{x}\right) x-S_{A}^{x} =0\\
\text{and \ } & \hat{S}_{A}^{y} z^{2} +\hat{S}_{A}^{y} zx+\left( S_{A}^{y} +F_{A}^{y} -\hat{S}_{A}^{y}\right) z-F_{A}^{y} =0.
\end{aligned}
\end{equation}
We can define $f_1(x,z)$ and $f_2(x,z)$ to be the left-hand sides of above equations and define $\mathbf{f} =( f_{1} ,f_{2})$, and then solve $\mathbf{f}( x,z) =0$ on $[ 0,1]^{2}$ by the Newton's method. 

==> backup/root_v1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%2345678901234567890123456789012345678901234567890123456789012345678901234567890
%        1         2         3         4         5         6         7         8

%%%%%%%%%%% change the following two lines for ICRA/R-AL formatting

% \input{00R-AL-header}
% \input{00ICRA-header}
\input{0_0Initial_submission_header}
% \newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}%[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\begin{document}



\maketitle
% \thispagestyle{empty}
% \pagestyle{empty}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{0_Abstract}

\input{1_Sections}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{INTRODUCTION}

% This template provides authors with most of the formatting specifications needed for preparing electronic versions of their papers. All standard paper components have been specified for three reasons: (1) ease of use when formatting individual papers, (2) automatic compliance to electronic requirements that facilitate the concurrent or later production of electronic products, and (3) conformity of style throughout a conference proceedings. Margins, column widths, line spacing, and type styles are built-in; examples of the type styles are provided throughout this document and are identified in italic type, within parentheses, following the example. Some components, such as multi-leveled equations, graphics, and tables are not prescribed, although the various table text styles are provided. The formatter will need to create these components, incorporating the applicable criteria that follow.

% \section{PROCEDURE FOR PAPER SUBMISSION}

% \subsection{Selecting a Template (Heading 2)}

% First, confirm that you have the correct template for your paper size. This template has been tailored for output on the US-letter paper size. 
% It may be used for A4 paper size if the paper size setting is suitably modified.

% \subsection{Maintaining the Integrity of the Specifications}

% The template is used to format your paper and style the text. All margins, column widths, line spaces, and text fonts are prescribed; please do not alter them. You may note peculiarities. For example, the head margin in this template measures proportionately more than is customary. This measurement and others are deliberate, using specifications that anticipate your paper as one part of the entire proceedings, and not as an independent document. Please do not revise any of the current designations

% \section{MATH}

% Before you begin to format your paper, first write and save the content as a separate text file. Keep your text and graphic files separate until after the text has been formatted and styled. Do not use hard tabs, and limit use of hard returns to only one return at the end of a paragraph. Do not add any kind of pagination anywhere in the paper. Do not number text heads-the template will do that for you.

% Finally, complete content and organizational editing before formatting. Please take note of the following items when proofreading spelling and grammar:

% \subsection{Abbreviations and Acronyms} Define abbreviations and acronyms the first time they are used in the text, even after they have been defined in the abstract. Abbreviations such as IEEE, SI, MKS, CGS, sc, dc, and rms do not have to be defined. Do not use abbreviations in the title or heads unless they are unavoidable.

% \subsection{Units}

% \begin{itemize}

% \item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as Ò3.5-inch disk driveÓ.
% \item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
% \item Do not mix complete spellings and abbreviations of units: ÒWb/m2Ó or Òwebers per square meterÓ, not Òwebers/m2Ó.  Spell out units when they appear in text: Ò. . . a few henriesÓ, not Ò. . . a few HÓ.
% \item Use a zero before decimal points: Ò0.25Ó, not Ò.25Ó. Use Òcm3Ó, not ÒccÓ. (bullet list)

% \end{itemize}


% \subsection{Equations}

% The equations are an exception to the prescribed specifications of this template. You will need to determine whether or not your equation should be typed using either the Times New Roman or the Symbol font (please no other font). To create multileveled equations, it may be necessary to treat the equation as a graphic and insert it into the text after your paper is styled. Number equations consecutively. Equation numbers, within parentheses, are to position flush right, as in (1), using a right tab stop. To make your equations more compact, you may use the solidus ( / ), the exp function, or appropriate exponents. Italicize Roman symbols for quantities and variables, but not Greek symbols. Use a long dash rather than a hyphen for a minus sign. Punctuate equations with commas or periods when they are part of a sentence, as in

% $$
% \alpha + \beta = \chi \eqno{(1)}
% $$

% Note that the equation is centered using a center tab stop. Be sure that the symbols in your equation have been defined before or immediately following the equation. Use Ò(1)Ó, not ÒEq. (1)Ó or Òequation (1)Ó, except at the beginning of a sentence: ÒEquation (1) is . . .Ó

% \subsection{Some Common Mistakes}
% \begin{itemize}


% \item The word ÒdataÓ is plural, not singular.
% \item The subscript for the permeability of vacuum ?0, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ÒoÓ.
% \item In American English, commas, semi-/colons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
% \item A graph within a graph is an ÒinsetÓ, not an ÒinsertÓ. The word alternatively is preferred to the word ÒalternatelyÓ (unless you really mean something that alternates).
% \item Do not use the word ÒessentiallyÓ to mean ÒapproximatelyÓ or ÒeffectivelyÓ.
% \item In your paper title, if the words Òthat usesÓ can accurately replace the word ÒusingÓ, capitalize the ÒuÓ; if not, keep using lower-cased.
% \item Be aware of the different meanings of the homophones ÒaffectÓ and ÒeffectÓ, ÒcomplementÓ and ÒcomplimentÓ, ÒdiscreetÓ and ÒdiscreteÓ, ÒprincipalÓ and ÒprincipleÓ.
% \item Do not confuse ÒimplyÓ and ÒinferÓ.
% \item The prefix ÒnonÓ is not a word; it should be joined to the word it modifies, usually without a hyphen.
% \item There is no period after the ÒetÓ in the Latin abbreviation Òet al.Ó.
% \item The abbreviation Òi.e.Ó means Òthat isÓ, and the abbreviation Òe.g.Ó means Òfor exampleÓ.

% \end{itemize}


% \section{USING THE TEMPLATE}

% Use this sample document as your LaTeX source file to create your document. Save this file as {\bf root.tex}. You have to make sure to use the cls file that came with this distribution. If you use a different style file, you cannot expect to get required margins. Note also that when you are creating your out PDF file, the source file is only part of the equation. {\it Your \TeX\ $\rightarrow$ PDF filter determines the output file size. Even if you make all the specifications to output a letter file in the source - if your filter is set to produce A4, you will only get A4 output. }

% It is impossible to account for all possible situation, one would encounter using \TeX. If you are using multiple \TeX\ files you must make sure that the ``MAIN`` source file is called root.tex - this is particularly important if your conference is using PaperPlaza's built in \TeX\ to PDF conversion tool.

% \subsection{Headings, etc}

% Text heads organize the topics on a relational, hierarchical basis. For example, the paper title is the primary text head because all subsequent material relates and elaborates on this one topic. If there are two or more sub-topics, the next level head (uppercase Roman numerals) should be used and, conversely, if there are not at least two sub-topics, then no subheads should be introduced. Styles named ÒHeading 1Ó, ÒHeading 2Ó, ÒHeading 3Ó, and ÒHeading 4Ó are prescribed.

% \subsection{Figures and Tables}

% Positioning Figures and Tables: Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be below the figures; table heads should appear above the tables. Insert figures and tables after they are cited in the text. Use the abbreviation ÒFig. 1Ó, even at the beginning of a sentence.

% \begin{table}[h]
% \caption{An Example of a Table}
% \label{table_example}
% \begin{center}
% \begin{tabular}{|c||c|}
% \hline
% One & Two\\
% \hline
% Three & Four\\
% \hline
% \end{tabular}
% \end{center}
% \end{table}


%   \begin{figure}[thpb]
%       \centering
%       \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
% }}
%       %\includegraphics[scale=1.0]{figurefile}
%       \caption{Inductance of oscillation winding on amorphous
%       magnetic core versus DC bias magnetic field}
%       \label{figurelabel}
%   \end{figure}
   

% Figure Labels: Use 8 point Times New Roman for Figure labels. Use words rather than symbols or abbreviations when writing Figure axis labels to avoid confusing the reader. As an example, write the quantity ÒMagnetizationÓ, or ÒMagnetization, MÓ, not just ÒMÓ. If including units in the label, present them within parentheses. Do not label axes only with units. In the example, write ÒMagnetization (A/m)Ó or ÒMagnetization {A[m(1)]}Ó, not just ÒA/mÓ. Do not label axes with a ratio of quantities and units. For example, write ÒTemperature (K)Ó, not ÒTemperature/K.Ó

% \section{CONCLUSIONS}

% A conclusion section is not required. Although a conclusion may review the main points of the paper, do not replicate the abstract as the conclusion. A conclusion might elaborate on the importance of the work or suggest applications and extensions. 

% \addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
%                                   % on the last page of the document manually. It shortens
%                                   % the textheight of the last page by a suitable amount.
%                                   % This command does not take effect until the next page
%                                   % so it should come on the page before the last. Make
%                                   % sure that you do not shorten the textheight too much.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section*{APPENDIX}

% Appendixes should appear before the acknowledgment.

%  \section*{ACKNOWLEDGMENT}


% The preferred spelling of the word ÒacknowledgmentÓ in America is without an ÒeÓ after the ÒgÓ. Avoid the stilted expression, ÒOne of us (R. B. G.) thanks . . .Ó  Instead, try ÒR. B. G. thanksÓ. Put sponsor acknowledgments in the unnumbered footnote on the first page.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.



% \begin{thebibliography}{99}

% \bibitem{c1} G. O. Young, ÒSynthetic structure of industrial plastics (Book style with paper title and editor),Ó 	in Plastics, 2nd ed. vol. 3, J. Peters, Ed.  New York: McGraw-Hill, 1964, pp. 15Ð64.
% \bibitem{c2} W.-K. Chen, Linear Networks and Systems (Book style).	Belmont, CA: Wadsworth, 1993, pp. 123Ð135.
% \bibitem{c3} H. Poor, An Introduction to Signal Detection and Estimation.   New York: Springer-Verlag, 1985, ch. 4.
% \bibitem{c4} B. Smith, ÒAn approach to graphs of linear forms (Unpublished work style),Ó unpublished.
% \bibitem{c5} E. H. Miller, ÒA note on reflector arrays (Periodical styleÑAccepted for publication),Ó IEEE Trans. Antennas Propagat., to be publised.
% \bibitem{c6} J. Wang, ÒFundamentals of erbium-doped fiber amplifiers arrays (Periodical styleÑSubmitted for publication),Ó IEEE J. Quantum Electron., submitted for publication.
% \bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
% \bibitem{c8} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ÒElectron spectroscopy studies on magneto-optical media and plastic substrate interfaces(Translation Journals style),Ó IEEE Transl. J. Magn.Jpn., vol. 2, Aug. 1987, pp. 740Ð741 [Dig. 9th Annu. Conf. Magnetics Japan, 1982, p. 301].
% \bibitem{c9} M. Young, The Techincal Writers Handbook.  Mill Valley, CA: University Science, 1989.
% \bibitem{c10} J. U. Duncombe, ÒInfrared navigationÑPart I: An assessment of feasibility (Periodical style),Ó IEEE Trans. Electron Devices, vol. ED-11, pp. 34Ð39, Jan. 1959.
% \bibitem{c11} S. Chen, B. Mulgrew, and P. M. Grant, ÒA clustering technique for digital communications channel equalization using radial basis function networks,Ó IEEE Trans. Neural Networks, vol. 4, pp. 570Ð578, July 1993.
% \bibitem{c12} R. W. Lucky, ÒAutomatic equalization for digital communication,Ó Bell Syst. Tech. J., vol. 44, no. 4, pp. 547Ð588, Apr. 1965.
% \bibitem{c13} S. P. Bingulac, ÒOn the compatibility of adaptive controllers (Published Conference Proceedings style),Ó in Proc. 4th Annu. Allerton Conf. Circuits and Systems Theory, New York, 1994, pp. 8Ð16.
% \bibitem{c14} G. R. Faulhaber, ÒDesign of service systems with priority reservation,Ó in Conf. Rec. 1995 IEEE Int. Conf. Communications, pp. 3Ð8.
% \bibitem{c15} W. D. Doyle, ÒMagnetization reversal in films with biaxial anisotropy,Ó in 1987 Proc. INTERMAG Conf., pp. 2.2-1Ð2.2-6.
% \bibitem{c16} G. W. Juette and L. E. Zeffanella, ÒRadio noise currents n short sections on bundle conductors (Presented Conference Paper style),Ó presented at the IEEE Summer power Meeting, Dallas, TX, June 22Ð27, 1990, Paper 90 SM 690-0 PWRS.
% \bibitem{c17} J. G. Kreifeldt, ÒAn analysis of surface-detected EMG as an amplitude-modulated noise,Ó presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
% \bibitem{c18} J. Williams, ÒNarrow-band analyzer (Thesis or Dissertation style),Ó Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
% \bibitem{c19} N. Kawasaki, ÒParametric study of thermal and chemical nonequilibrium nozzle flow,Ó M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
% \bibitem{c20} J. P. Wilkinson, ÒNonlinear resonant circuit devices (Patent style),Ó U.S. Patent 3 624 12, July 16, 1990. 


\bibliographystyle{IEEEtran}
\bibliography{reference}
% \printbibliography


% \end{thebibliography}




\end{document}


==> backup/sections_v1.tex <==
\section{Introduction}\label{sec:intro}
Human-autonomy teaming is a major focus in the ongoing transformation of future workplace. To enable effective teaming, trust has been identified as one central factor. Despite the research efforts over the past thirty years, existing literature is predominantly focused on dyadic human-autonomy teams where one human agent interacts with one autonomous agent. There is little, if not no, understanding on how to model the evolution of trust in teams consisting of multiple human agents and multiple autonomous agents. 


% To fill the above research gaps, this study aims to model trust dynamics in MOMA interaction wherein multiple humans interacts with multiple autonomous agents.

Consider a scenario where two human agents, $x$ and $y$, and two autonomous agents, $A$ and $B$ are to perform a task. The four agents are allowed to form sub-teams to enhance task performance (e.g., maximizing throughput, minimizing task completion time). For example, they could form two dyadic human-robot teams to complete certain part of the task, and later decides to merge the two sub-teams to complete other parts of the task. 

Here exist two types of experiences that an human agent may have with an autonomous agent: direct and indirect experience. Direct experience, by its name, means a human agent's interaction with an autonomous agent is through him-/her-self; In-direct experience means a human agent's interaction with an autonomous agent is mediated by another party, for example, another human agent. In Fig~\ref{fig:trust-transfer}, human $x$ works directly with robot $B$ and human $y$ works directly with robot $A$. Even though there is no direct interaction between $x$ and $A$, we postulate that $x$ could still establish his or her trust on $A$ by learning $y$'s trust towards $A$, i.e., $y$'s trust in $A$ propagate to $x$. 


Trust modeling in dyadic human-robot teams focuses on examining how direct experience influences a human agent's trust in a robot. Real-time trust estimators based on direct interaction has been proposed and compared (CITE). In multi-human multi-robot teams, we postulate that \textit{both direct and indirect interaction drive a human agent's trust in an autonomous agent}. 
% To model trust dynamics in MOMA team, we propose a trust updating model based on both the direct and indirect interaction. 


% Trust influences a human's reliance on a robot~\cite{lewandowsky2000dynamics, muir1996trust} and thus has been identified as a crucial factor in human-robot interaction (HRI). For example, either distrust or overtrust would lead to inefficient human-robot collaboration~\cite{lewis2018role}.

% As a result, trust in HRI has attracted much research interest, including traditional work on antecedents and consequences of trust in robots and recent work on trust-aware interaction algorithms~\cite{kok2020trust}.  

% However, most of these studies focus on direct human-robot trust, and limited research has been done on trust propagation in a multi-agent human-robot team. 


% Here, the term \textit{direct trust} refers to the trust gained via direct interaction, while

% We define \textit{trust propagation} the process of adjusting one's trust in a robot by learning a third party's trust on the robot. Fig~\ref{fig:trust-transfer} provides a schematic view: human $x$ works directly with robot $B$ and human $y$ works directly with robot $A$. Even though there is no direct interaction between $x$ and $A$, $x$ could still establish his or her trust $t^x_A$ on $A$ by referring to $y$'s trust towards $A$. If robot $A$ is running a trust-aware algorithm that needs to estimates the trust $t^x_A$, then $A$ must understand how trust propagation works. In fact, many trust propagation models have been developed as they are essential to trust management~\cite{urena2019review}. However, a majority of these models were proposed for large-scale online platforms, such as e-commerce~\cite{cen2019trust, jiang2019trust} and social networks~\cite{fan2019graph}, and thus don't necessarily agree with empirical findings on trust in robots. Therefore, a trust propagation model is necessary for the future research on trust-aware HRI.

% With the increasing trend towards multi-agent HRI research~\cite{schneiders2022non}, a trust propagation model is necessary for future research on trust-aware HRI.

\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{figs/transition-illustration.pdf}
  \caption{$x$ may need to refer to $y$'s trust $t^y_B$ to establish his or her trust $t^x_B$ on $B$ through trust propagation.}
  \label{fig:trust-transfer}
\end{figure}

In this study, we develop a novel trust inference and propagation (TIP) model for multi-human multi-robot teams, explicitly accounting for the direct and indirect experience a human agent may have with an autonomous agent. 
% In the model, a human agent adjust his or her trust in an autonomous agent through two types of interactions. The first type is direct trust update, where a human works directly with a robot and updates his or her trust directly based on the interaction experience; the second type is the indirect trust update, where a human agent updates his or her trust by learning a third party's trust in the autonomous agent (i.e., the third party's trust propagates to the human agent). We studied the proposed model using a human-subject experiment. 
% Results show that in both direct-only trust update and mixed trust update the trust value will stabilize after enough interactions. 
To evaluate the proposed TIP model, we conducted a human-subject experiment with 11 pairs of participants.  Each pair worked with two drones to perform a search task at 15 sessions. In one session, one human agent in the pair works with one drone randomly assigned to them. At the end of each session the pair communicate with each other their trust in the robot they just interacted with. Results from the experiment indicate that over time, the two human agent's trust toward each robotic agent converges, supporting the existence of trust propagation between humans. Moreover, we compared the proposed the TIP model with a direct-experience-only model where only direct interaction influences the human agent's trust. Results indicate that the proposed TIP model successfully captured the behavior of trust in a multi-agent human-robot team, with a significantly smaller RMSE compared to the direct-experience-only model, .

% To fill this research gap, in this work, we proposed the TRUP\footnote{TRUP stands for \textbf{Tru}st \textbf{p}ropagation}, an innovative trust propagation model for human-robot interaction. In the model, trust evolves through two types of interactions. The first type is direct trust update, where a human works directly with a robot and updates his or her trust directly based on the interaction experience; the second type is the indirect trust update, where a human updates his or her trust by comparing it to a third party's trust. We studied the behavior of the TRUP model under repeated interactions. Results show that in both direct-only trust update and mixed trust update the trust value will stabilize after enough interactions. Additionally, we conducted a human-subject experiment to evaluate our model. We designed an experiment wherein two participants take turns to work with two robots on a threat-detection task. The two participants in the same group can communicate their trust with each other. Results show that the within-group trust difference on each robot is significantly smaller than the between-group trust difference, supporting the existence of trust propagation between humans. Fitting results showed the proposed model successfully captured the behavior of trust in a multi-agent human-robot team.

The contributions of this work include: 
\begin{itemize}
    \item We demonstrate the existence of trust propagation from one human agent to another in a multi-human multi-robot team.
    \item To the best of our knowledge, the proposed TIP is the first mathematical formulation that accounts for both the direction experience and indirect experiences (through propagation) a human agent may have with an autonomous agent in multi-human multi-robot teams. 
    \item We conduct a human-subject experiment to assess the proposed model. Results show superior performance of the TIP model in capturing each human agent's real-time trust in each autonomous agent in a multi-human multi-robot team.  

\end{itemize}


This paper is organized as follows: in Section~\ref{sec:relatedWork}, we discuss the related work, including computational trust models in HRI and trust propagation models in other fields; in Section~\ref{sec:model}, we introduce the mathematical formulation of the TRUP model and study its behavior under different types of interactions; in Section~\ref{sec:humanStudy}, we present the human-subject study and the fitting results; Section~\ref{sec:discussion} contains discussions.

\section{Related Work}\label{sec:relatedWork}
In this section, we first briefly review the relevant work on trust in automation, including the trust dynamics, computational trust models, and trust propagation models. 

As trust is extensively studied in many fields, it has been given different definitions~\cite{cho2015survey}. In this work, we focus on trust in automation and use the definition given by Lee and See~\cite{See:2004vj}, which defines trust as ``the attitude that an agent will help achieve an individual’s goals in situations characterized by uncertainty and vulnerability". This definition emphasizes the uncertain nature of HRI and the vulnerability of a human trusting a robot in collaborations and therefore serves our purpose.

\subsection{Trust Dynamics and Modeling}
Trust dynamics include the factors affecting trust and how trust is affected. Based on the work of Lee and Moray~\cite{lee1992trust}, the robot-related factors can be further classified into three categories: performance, process, and purpose, where performance refers to the automation's ability to complete the task, process refers to how the automation operates, and purpose describes the intent of the automation. Previous studies on modeling trust in robots assumed robots are not deceptive and took a performance-centric approach~\cite{chen2018planning, desai2012modeling, Xu2015optimo, wang2016impact, Guo2020_IJSR, pippin2014trust}. Empirical studies have shown a robot's performance affects trust in two feedback loops, namely a positive and a negative feedback loop~\cite{manzey2012human}. The positive loop is caused by automation success while the negative loop is caused by automation failure, where the negative one has a stronger effect than the positive one~\cite{lee1992trust, yang2016users}. Yang et al.~\cite{yang2017evaluating} examined how trust evolved when an average human agent interacts with a robot. They showed that the trust stabilized over repeated interactions. In their later work~\cite{yangtrust2022}, Yang et al. suggested three properties of trust dynamics that resulted from performance, namely continuity, negativity bias, and stabilization. 

Several computational models of trust in robots exist in literature. Xu and Dudek~\cite{Xu2015optimo} proposed the online probabilistic trust inference model (OPTIMo) utilizing Bayesian networks to estimate human trust from automation's performance and human behavior. Hu et al.~\cite{hu2016real} proposed to predict binary-valued trust, i.e., trust or distrust, based on human's electroencephalography (EEG) and galvanic skin response (GSR) data. Lu and Sarter~\cite{Lu2020} compared logistic regression, k-Nearest Neighbors (kNN), and random forest in predicting human trust using real-time eye-tracking data. Soh et al.~\cite{soh2020multi} modeled trust as a latent dynamic function for predicting human trust in robots across different tasks. Guo and Yang~\cite{Guo2020_IJSR} proposed to model trust as a Beta random variable and predict trust value in a Bayesian framework.



% Lee and Moray~\cite{lee1992trust} proposed the auto-regressive moving average vector (ARMAV) model where trust is computed as as a function of task performance and the occurrence of automation failures. 


% In this work, we use the trust model proposed by Guo and Yang~\cite{Guo2020_IJSR}, where trust is modeled as a Beta distribution characterized by positive and negative interaction experiences. This Beta distribution model adheres to three important properties of trust dynamics \cite{Yang:2021}, namely, \textit{continuity}, \textit{negativity bias}, and \textit{stabilization}, thus providing good model predictability, explicablity, and generalizability. 
%Hancock et al.~\cite{hancock2021evolving} analyzed empirical findings on the antecedents of trust in robots and classified them into three categories, including human, robot, and environmental sources.
% Manzey et al.~\cite{manzey2012human} suggested that a robot's performance affects trust in two feedback loops, namely a positive and a negative feedback loop. The positive loop is caused by automation success while the negative loop is caused by automation failure, where the negative one has a stronger effect than the positive one~\cite{lee1992trust, yang2016users}. Yang et al.~\cite{yang2017evaluating} examined how trust evolved when an average human agent interacts with a robot. They showed that the trust stabilized over repeated interactions. In the following work~\cite{yangtrust2022}(\textcolor{green}{is this citation published?}), Yang et al. suggested three properties of trust dynamics resulted from performance, namely continuity, negativity bias, and stabilization.

\subsection{Trust Propagation Models}
Trust propagation models are developed to estimate the unknown trust value between two agents using existing trust relations. They are primarily used as modules for trust or reputation management systems in multi-agent platforms, especially in the flow reputation system~\cite{hendrikx2015reputation}, where trust can propagate through the network. For example, Jøsang proposed a formal framework of trust called subjective logic~\cite{josang1997artificial} and later incorporated it in the Beta reputation system~\cite{josang2002beta}. According to subjective logic, the trust of an individual towards another is represented as a tuple called opinion, which consists of belief, disbelief, and uncertainty, and opinions can transfer through individuals by the discounting rule. Another example is the FIRE trust management model proposed by Huynh et al.~\cite{huynh2004fire}, where they used the term "witness reputation" as one's transitive trust. One's witness reputation is calculated as a weighted sum of trust values from its connected neighbors.
% A common feature in the existing trust propagation models is the amount of transferred trust is  the more an agent trusts another, the more trust will be transferred. 
Variants of such propagation mechanisms can be found in several multi-agent systems, such as e-commerce~\cite{cen2019trust, jiang2019trust} and social networks~\cite{fan2019graph}.



\section{Mathematical Model}\label{sec:model}
We present the detailed TRUP model. Our key motivation is to develop a fully computational trust propagation model that works in general HRI settings and agrees with the empirical findings of trust in robots. We first discuss the assumptions we made, and then present the mathematical formulation, and finally examine the behavior of the model under repeated human-robot interactions.  


\subsection{Assumptions}\label{subsec:assumptions}
We make two major assumptions in the context of HRI. First, we assume that \textit{each human agent communicates trust as a single-dimensional random variable}. In some work, trust is represented as a tuple. For example, in~\cite{josang2002beta}, trust consists of a triplet, i.e., belief, disbelief, and uncertainty. Although a multi-dimensional representation can convey more information, in human-robot teams, it is impractical to assume human agents communicate trust in such a manner because keeping track of multiple numbers adds mental load and may not be pragmatic for non-experts.
%Therefore, we assume a simple one-dimension form of trust to fit our model in a general HRI context.

Second, we assume that \textit{human agents are cooperative}, i.e., they are honest and share the same goal. With this assumption, the human agents always communicate their true trust to each other to their best ability and hence we do not need a model to further process the communicated trust.

% According to Mayer et al., the bases of trust include the trustee's ability, integrity,and benevolence~\ref{mayer1995integrative}. With the cooperation assumption, an human agent's ability is the only factor affecting how another agent trusts him or her. 


% trustee's integrity and benevolence are consistent, and thus the trustor's trust evolves only when the trustor's perceived ability of the trustee changes. Moreover, as the trustee is honest, when he or she informs the trustor of his or her trust on a robot, the trustor will possibly discount, but not try to reverse, this information. For example, if $y$ tells $x$ that robot $A$ is \%90 trustworthy, then $x$ may think 


% Under the second assumption, the trustor establishes his or her trust only through the trustee's ability. Furthermore, in the context of trust propagation, this ability refers to the trustee's ability of 'correctly' rating a trust Moreover, 


% Among these factors, robot's performance is often more accessible to the human teammates. Therefore, similar to previous studies~\cite{chen2018planning, desai2012modeling, Xu2015optimo, wang2016impact, Guo2020_IJSR}, we consider the performance of a robot as the major antecedent of trust. 

\subsection{Proposed Model}
% \textcolor{green}{better notation?}
\textbf{Trust as a Beta random variable}: We take a probabilistic view to model trust. At time $k$, the trust $t_{k}^{a,b}$ that a human agent $a$ feels towards another agent $b$ follows a Beta distribution, i.e., 
\begin{equation} \label{eq:trust_def} 
% t_{b}^{a} (k)\sim \operatorname{Beta}\left( \alpha _{b}^{a} (k),\beta _{b}^{a} (k)\right)
t_{k}^{a,b} \sim \operatorname{Beta}\left( \alpha _{k}^{a,b} ,\beta _{k}^{a,b}\right)
\text{,}
\end{equation}
where $\alpha _{k}^{a,b}$ and $\beta _{k}^{a,b}$ are the positive and negative experiences $a$ had about $b$ up to time $k$, respectively. Correspondingly, the expected trust is given by
\begin{equation} \label{eq:trust_expected} 
\mu _{k}^{a,b} =\alpha _{k}^{a,b} /\left( \alpha _{k}^{a,b} +\beta _{k}^{a,b}\right)
\text{.}
\end{equation}
Here we note that $t_{k}^{a,b}$ is the queried trust given by the agent $a$, which has some randomness due to subjectivity, while $\mu_{k}^{a,b}$ is the expected trust determined by the experiences.

% Eq.~\eqref{eq:trust_def} captures the characteristics of trust that human trust is affected by interaction experiences and gaining experiences decreases the variance of trust. 
% Note that agent $b$ here can be either a human agent or a robot agent, and hence the definition applies to both human-to-human trust and human-to-robot trust.

\smallskip
\textbf{Trust update through direct experience:} Similar to~\cite{Guo2020_IJSR}, we update the direct trust experience at time ${k}$ by setting 
\begin{equation}\label{eq:direct_update}
\begin{aligned}
\alpha _{k}^{a,b} & =\alpha _{k-1}^{a,b} +s^{a,b} \cdot p_{k}^{b}\\
\beta _{k}^{a,b} & =\beta _{k-1}^{a,b} +f^{a,b} \cdot \overline{p}_{k}^{b}
% \alpha _{b}^{a} (k) & =\alpha _{b}^{a} (k-1)+s_{b}^{a} \cdot p_{b} (k)\\
% \beta _{b}^{a} (k) & =\beta _{b}^{a} (k-1)+f_{b}^{a} \cdot \overline{p}_{b} (k)
\end{aligned}\text{.}
\end{equation}
Here $p_{k}^{b}$ and $\overline{p}_{k}^{b}$ are the measurements of $b$'s success and failure during time $k$; and, $s^{a,b}$ and $f^{a,b}$ are $a$'s unit experience gains with respect to success or failure of $b$. We require $s^{a,b}$ and $f^{a,b}$ to be positive to ensure that cumulative experiences are non-decreasing. The updated trust $t_{k}^{a,b}$ follows the distribution $\operatorname{Beta}\left( \alpha _{k}^{a,b} ,\beta _{k}^{a,b}\right)$.

\smallskip
\textbf{Trust update through indirect experience propagation:} Let $x$ and $y$ denote two human agents and let $A$ denote a robot agent, as illustrated in Fig.~\ref{fig:trust-transfer}. At time $k$, $y$ communicates his or her trust $t_{k}^{y,A}$ on $A$ with $x$, and then $x$ updates his or her indirect trust experience by 
\begin{equation}\label{eq:indirect_update}
\begin{aligned}
\alpha _{k}^{x,A} & =\alpha _{k-1}^{x,A} +t_{k}^{x,y} \cdot \hat{s}^{x,A} \cdot \left[ t_{k}^{y,A} -\mu _{k-1}^{x,A}\right]^{+}\\
\beta _{k}^{x,A} & =\beta _{k-1}^{x,A} +t_{k}^{x,y} \cdot \hat{f}^{x,A} \cdot \left[ \mu _{k-1}^{x,A} -t_{k}^{y,A}\right]^{+}
% \alpha _{A}^{x} (k) & =\alpha _{A}^{x} (k-1)+t_{y}^{x} (k)\cdot \hat{s}_{A}^{x} \cdot \left[ t_{A}^{y} (k)-t_{A}^{x} (k-1)\right]^{+}\\
% \beta _{A}^{x} (k) & =\beta _{A}^{x} (k-1)+t_{y}^{x} (k)\cdot \hat{f}_{A}^{x} \cdot \left[ t_{A}^{x} (k-1)-t_{A}^{y} (k)\right]^{+}
\end{aligned}\text{,}
\end{equation}
where the superscript $+$ means the positive part of the corresponding number, i.e., $t^+=\max\{0,t\}$ for a real number $t$, and $t_{k}^{x,A}\sim \operatorname{Beta}\left( \alpha _{k}^{x,A} ,\beta _{k}^{x,A}\right)$. The intuition behind this model is that $x$ needs to reason upon $t_{k}^{y,A}$, i.e., $y$'s trust towards $A$. First, $x$ compares $y$'s trust $t_{k}^{y,A}$ with his or her own expected trust $\mu_{k-1}^{x,A}$. Let $\Delta t:=t_{k}^{y,A} -\mu_{k-1}^{x,A}$ be the difference. If $\Delta t \ge 0$, $x$ gains positive indirect experience about $A$, which amounts to the product of the trust difference $\Delta t$, a coefficient $\hat{s}^{x,A}$, and a discounting factor $t_{k}^{x,y}$, i.e., $x$'s trust on $y$; if $\Delta t<0$, then $x$ gains negative indirect experience about $A$, which is defined similarly. 

\subsection{Asymptotic Behavior under Repeated Interactions}
We examine the behavior of the proposed model under both direct and indirect interactions. Consider a scenario where human agents $x$ and $y$ take turns to work with robot $A$ repetitively. Suppose each $x$'s turn contains $m$ interactions while each $y$'s turn contains $n$ interactions; and, after each interaction, the agent who works directly with $A$ informs the other agent of his or her trust on $A$. Fig.~\ref{fig:repetitive_interactions} illustrates the interaction process. In addition, we assume that robot $A$ has constant reliability $r$, i.e., $A$'s performance measure are $p_{k}^A =r$ and $\overline{p}^{A}_k = \bar{r}$, for $k=1,2,...$, where $\bar{r}:=1-r$, and $x$ has constant trust $t_{y}^{x}$ in $y$. We only consider the case when $m$ and $n$ are not both zero since otherwise the case becomes trivial. Without loss of generality, we assume $m>0$ and $n\geqslant0$.
% study two possible cases for $x$. The proofs can be found in the appendix.
\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{figs/repetitive-interactions.pdf}
  \caption{$x$ and $y$ take turns to interact with $A$.}
  \label{fig:repetitive_interactions}
\end{figure}

% The following theorem states that both $t_{k}^{x,A}$ and $t_{k}^{y,A}$ stabilize after enough interactions. 
We have the following main result on the asymptotic behavior of $t_{k}^{x,A}$ and $t_{k}^{y,A}$.
\begin{theorem}
\label{thm:both_converge}
When $m >0$ and $n\geqslant 0$, $t_{k}^{x,A}$ and $t_{k}^{y,A}$ converge in probability (i.p.) respectively, i.e., there exists $t^{x}$ and $t^{y}$ such that, for any $\epsilon  >0$,
\begin{equation}
\begin{aligned}
 &  & \lim _{k\rightarrow \infty } \Pr\left(\left| t_{k}^{x,A} -t^{x}\right|  >\epsilon \right) =0\ \\
\text{and} &  & \lim _{k\rightarrow \infty } \Pr\left(\left| t_{k}^{y,A} -t^{y}\right|  >\epsilon \right) =0.
\end{aligned}
\end{equation}
\end{theorem}
This result exhibits that, under alternating interactions with the robot, both agents' trust will stabilize after enough interactions. In the next result, we give a method to compute the equilibria:

\begin{theorem}
\label{thm:equilibria}  
The equilibria $t^{x}$ and $t^{y}$ in Theorem~\ref{thm:both_converge}  satisfy
\begin{equation}
\label{eq:equilibria_case1}
\begin{aligned}
S^{x}\frac{1-t^{x}}{t^{x}} & =\hat{F}^{x}\left( t^{x} -t^{y}\right) +F^{x} & \text{and}\\
F^{y}\frac{t^{y}}{1-t^{y}} & =\hat{S}^{y}\left( t^{x} -t^{y}\right) +S^{y} & 
\end{aligned}
\end{equation}
if $S^{x} F^{y} \geqslant F^{x} S^{y}$; otherwise, they satisfy
\begin{equation}
\label{eq:equilibria_case2}
\begin{aligned}
F^{x}\frac{t^{x}}{1-t^{x}} & =\hat{S}^{x}\left( t^{y} -t^{x}\right) +S^{x} & \text{and}\\
S^{y}\frac{1-t^{y}}{t^{y}} & =\hat{F}^{y}\left( t^{y} -t^{x}\right) +F^{y} , & 
\end{aligned}
\end{equation}
where $\hat{S}^{x} =nt^{x,y}\hat{s}^{x,A}$, $\hat{F}^{x} =nt^{x,y}\hat{f}^{x,A}$, $S^{x} =ms^{x,A} r$, $F^{x} =mf^{x,A}\overline{r}$, $\hat{S}^{y} =mt^{y,x}\hat{s}^{y,A}$, $\hat{F}^{y} =mt^{y,x}\hat{f}^{y,A}$, $S^{y} =ns^{y,A} r$, and $F^{y} =nf^{y,A}\overline{r}$.
\end{theorem}
The capitalized variables in Theorem~\ref{thm:equilibria} are related to the average experience gains in the long run, e.g., ${S}^{x}$ is $x$'s direct positive experience gain after each $m$ direct interactions. The condition $S^{x} F^{y} \geqslant F^{x} S^{y}$ cab be interpreted as that, compared with $y$, $x$ tends to have a higher trust on $A$ after each direct interaction. $t^x$ and $t^y$ can be computed exactly by solving a cubic equation or approximated by the Newton's method. Details are given in the appendix.

When $n=0$, agent $x$ only updates trust on $A$ directly and agent $y$ only updates trust indirectly. Theorem~\ref{thm:equilibria} leads to the following corollary.
\begin{corollary}
\label{thm:converge_n=0}
When $m >0$ and $n=0$, $x$'s trust $t_{k}^{x,A}$ on $A$ converges to $t^{x} =\frac{s^{x,A} r}{f^{x,A}\overline{r} +s^{x,A} r}$ in probability, i.e., for any $\epsilon  >0$,
\begin{equation}
\lim _{k\rightarrow \infty } \Pr\left(\left| t_{k}^{x,A} -\frac{s^{x,A} r}{f^{x,A}\overline{r} +s^{x,A} r}\right|  >\epsilon \right) =0.
\end{equation}
The difference between $t_{k}^{x,A}$ and $t_{k}^{y,A}$ converge to 0 in probability, i.e., for any $\epsilon  >0$,
\begin{equation}
\lim _{k\rightarrow \infty } \Pr\left(\left| t_{k}^{x,A} -t_{k}^{y,A}\right|  >\epsilon \right) =0.
\end{equation}
Equivalently, we have $t^{x} =t^{y}$.
\end{corollary}

This result implies that, first, under direct-only trust updates, $x$'s trust will stabilize around $\frac{s^{x,A} r}{f^{x,A}\overline{r} +s^{x,A} r}$, which is determined by $s^{x,A}$ and $f^{x,A}$, $x$'s unit experience gains via direct trust, and $r$, the robot's reliability; second, under indirect-only updates, $y$'s trust will converge to $x$'s trust.




\subsection{Parameter Inference}
A human agent's trust on a robot is characterized by six parameters. For instance, the parameter set, denoted as $\theta ^{x,A}$, of $x$ on robot $A$ include $x$'s prior experiences $\alpha _{0}^{x,A}$ and $\beta _{0}^{x,A}$, the unit direct experience gains $s_{A}^{x}$ and $f_{A}^{x}$, and the unit indirect experience gains $\hat{s}_{A}^{x}$ and $\hat{f}_{A}^{x}$. Denote the indices of $x$'s direct and indirect interactions with $A$ upto time $k$ as $D_{k}$ and $\overline{D}_{k}$ respectively. Then, we can compute $\alpha _{k}^{x,A}$ and $\beta _{k}^{x,A}$, according to Eq.~\eqref{eq:direct_update} and Eq.~\eqref{eq:indirect_update}, as
\begin{equation}
\label{eq:alpha_k_beta_k}
\begin{aligned}
\alpha _{k}^{x,A} = & \alpha _{0}^{x,A} +s^{x,A}\sum _{j\in D_{k}} p_{j}^{A} +\hat{s}\sum _{j\in \overline{D}_{k}} t_{j}^{x,y}\left[ t_{j}^{y,A} -\mu _{j-1}^{x,A}\right]^{+}\\
\beta _{k}^{x,A} = & \beta _{0}^{x,A} +f^{x,A}\sum _{j\in D_{k}}\overline{p}_{j}^{A} +\hat{f}\sum _{j\in \overline{D}_{k}} t_{j}^{x,y}\left[ \mu _{j-1}^{x,A} -t_{j}^{y,A}\right]^{+}
\end{aligned} ,
\end{equation}
where $\mu \textcolor[rgb]{0,0,0}{_{j-1}^{x,A}}$ is the expectation of $t_{j-1}^{x,A}$ defined in \eqref{eq:trust_expected}. We compute the optimal parameter $\theta {^{x,A}}^{*}$ by maximum likelihood estimation (MLE), i.e., 
\begin{equation*}
\begin{aligned}
\theta {^{x,A}}^{*} = & \arg\max\log\Pr\left(\text{data}\middle| \theta ^{x,A}\right)\\
= & \arg\max\sum _{k=0}^{K}\log\operatorname{Beta}\left( t_{k}^{x,A}\middle| \alpha _{k}^{x,A} ,\beta _{k}^{x,A}\right)\text{.}
\end{aligned}
\end{equation*}
In particular, we formulate the parameter inference problem as follows: given $x$'s trust on $A$, $t_{k}^{x,A}$, $A$'s performance during direction interaction, $p_{k}^{A}$ and $\overline{p}_{k}^{A}$, $x$'s trust on $y$, $t_{\overline{k}}^{x,y}$, and $y$'s trust on $A$ during $x$'s indirect interaction, $t_{\overline{k}}^{y,A}$, for $k\in D_{k}$ and $\overline{k} \in \overline{D}_{k}$, $k=1,2,\dotsc ,K$, we want find the parameter set $\theta ^{x,A}$ that maximizes the log likelihood function
\begin{equation}
\label{eq:likelihood_def}
H\left( \theta ^{x,A}\right) :=\sum _{k=0}^{K}\log\operatorname{Beta}\left( t_{k}^{x,A}\middle| \alpha _{k}^{x,A} ,\beta _{k}^{x,A}\right) ,
\end{equation}
where $\alpha _{k}^{x,A}$ and $\beta _{k}^{x,A}$ are computed by \eqref{eq:alpha_k_beta_k}.

Unfortunately, $H$ is not concave due to the quotient involved in $\mu _{k}^{x,A}$. To work around, we approximate $\mu _{k}^{x,A}$ with $t_{k}^{x,A}$ and define the approximated experiences as 
\begin{equation}
\label{eq:alpha_k_beta_k_app}
\begin{aligned}
\tilde{\alpha }_{k}^{x,A} = & \tilde{\alpha }_{0}^{x,A} +s^{x,A}\sum _{j\in D_{k}} p_{j}^{A} +\hat{s}\sum _{j\in \overline{D}_{k}} t_{j}^{x,y}\left[ t_{j}^{y,A} -t_{j-1}^{x,A}\right]^{+}\\
\tilde{\beta }_{k}^{x,A} = & \tilde{\beta }_{0}^{x,A} +f^{x,A}\sum _{j\in D_{k}}\overline{p}_{j}^{A} +\hat{f}\sum _{j\in \overline{D}_{k}} t_{j}^{x,y}\left[ t_{j-1}^{x,A} -t_{j}^{y,A}\right]^{+}
\end{aligned} ,
\end{equation}
where $\tilde{\alpha }_{0} :=\alpha _{0}$ and $\tilde{\beta }_{0} :=\beta _{0}$; and, define the approximated log likelihood function as
\begin{equation}
\label{eq:likelihood_app_def}
\tilde{H}\left( \theta ^{x,A}\right) :=\sum _{k=0}^{K}\log\operatorname{Beta}\left( t_{k}^{x,A}\middle| \tilde{\alpha }_{k}^{x,A} ,\tilde{\beta }_{k}^{x,A}\right) .
\end{equation}

\begin{theorem}
\label{thm:bound_inference_optimum}
Let $\tilde{\theta }^{*} =\arg\max\tilde{H}( \theta )$ and $\theta ^{*} =\arg\max H( \theta )$. Then, for any $\epsilon  >0$,
\begin{equation}
\Pr\left(\left| H_{1}\left(\tilde{\theta }^{*}\right) -\log L\left( \theta ^{*}\right)\right|  >\epsilon '\right) < \frac{1}{\epsilon }\sum _{k\in \overline{D}_{K}}\frac{\alpha _{k-1} \beta _{k-1}}{(\alpha _{k-1} +\beta _{k-1} )^{3}}
\end{equation}
where 
\begin{equation}
\epsilon '=( S_{K} +T_{K})\sqrt{\epsilon } +\kappa \left(\mathbf{x}_{1} ,\tilde{\mathbf{x}}_{1}\right) \epsilon +\sum _{k=0}^{K}\left(\left| \tilde{R}\left(\tilde{\mathbf{x}}_{k}\right)\right| +\left| \tilde{R}(\mathbf{x}_{k})\right| \right) ,
\end{equation}
and 
\begin{equation}
\begin{aligned}
T_{K} & =\left(\sum _{k=0}^{K}\left[\log t{_{k}^{x,A}}^{2} +\log\left( 1-t_{k}^{x,A}\right)^{2}\right]\right)^{1/2}\\
S_{K} & =\sqrt{\sum _{k=0}^{K} \xi (\mathbf{x}_{k})^{2}}\\
\xi (\mathbf{x}) & =\sqrt{\frac{b}{a} +\frac{a}{b}} +\frac{1}{2( a +b)}\sqrt{\left(\frac{b}{a}\right)^{2} +\left(\frac{a}{b}\right)^{2}}\\
\varkappa ( a) & =\frac{1}{a} +\frac{1}{2a^{2}}\\
\kappa (\mathbf{x}_{1} ,\mathbf{x}_{2}) & =\frac{1}{2}\max\{\varkappa ( a_{1}) ,\varkappa ( b_{1}) ,\varkappa ( a_{2}) ,\varkappa ( b_{2})\}
\end{aligned} .
\end{equation}
\end{theorem}



\section{Human Subject Study}\label{sec:humanStudy}
We conducted a human-subject experiment to test the effectiveness of the proposed model in fitting multi-agent human-robot trust data. The experiment, inspired by~\cite{yang2017evaluating}, simulated a threat-detection task, where two human agents work with two smart drones alternatively to search threats in multiple sites.   

\subsection{Experiment Design}
In the experiment, a group of two participants were asked to conduct a simulated threat-detection mission with two assistant drones for 15 sessions on two separated desktop computers. At each session, each participant was assigned with one drone and then worked on the detection tasks. At the end of each session, they were asked to report their trust values. To study trust propagation, we collected two types of trust: the first type was each participant's trust towards each drone, which was based on how much he or she trusted the drone to perform the detection task; the second type was each participant's trust towards the other participant, which was based on how much they would trust on the other participant's ability to rate trust on the drones. For the sake of clarity, we named the drones as drone $A$ and drone $B$ and colored them in red and blue respectively; and, we denoted the participants as $x$ and $y$ respectively. A trust rating is denoted as $t^a_b(k)$, where the superscript $a\in \{x,y\}$ stands for the trustor, the subscript $b\in \{x,y,A,B\}$ stands for the trustee, and $k$ denotes the session index. For example, $t^x_A(2)$ is the trust rating given by participant $x$ on the drone $A$ after the second session. The range of a trust rating is $[0,1]$, where 0 stands for not trust at all and 1 stands for completely trust.  
\input{fig_experiment_design}

The experiment process is illustrated in Fig.~\ref{fig:process}, which includes four major parts:

\textbf{Initial trust rating}: At the start, each participant gave their initial trust in the two drones based on their previous experience with automation. Additionally, they gave their initial trust towards each other. These trust ratings were indexed by 0, e.g., $x$'s initial trust rating on $A$ was denoted as $t^x_A(0)$

\textbf{Robot assignment}: At the beginning of each session, each participant was randomly assigned with one drone as his or her assistant robot.

\textbf{Detection task}: Each session consisted of 10 locations to detect. As shown in Fig.~\ref{fig:interface}, four views were present at each location. If a threat, which appeared like enemy combatants, was in any of the views, the participant should click the `Danger' button; otherwise, they should click the `Clear' button. Meanwhile, his or her drone would highlight the background of a view if it detected a threat there. In addition, a 2-second timer was set for each location. If a participant didn't click either button before the timer counted down to zero, the testbed
% would mark his or her detection result as wrong for the current location and then 
would go to the next location automatically. After all the 10 locations, an end-of-session screen was shown, displaying how many correct choices the participant and the drone had made in the current session respectively. Here the rule was that, at each location, a participant's choice would be marked as wrong if he or she clicked the wrong button or didn't click either button before time was out; otherwise, it was marked as correct. For the drone, its choice was wrong if its detection result was wrong, e.g., if there was no threat but it highlighted a view.

\textbf{Trust rating}: After each session, the testbed asked for several trust ratings from the participants, as shown in Fig.~\ref{fig:trust-rating}. First, each participant gave his or her \textit{direct trust update}, i.e., to adjust the trust rating on the drone s/he just worked with in the current session. Next, the system showed these direct trust ratings to both the participants and asked for their \textit{indirect trust update}, e.g., each participant's trust rating on the drone that he or she didn't work with in the current session. Finally, the participants updated their trust towards each other. If the participants had completed all 15 sessions, the experiment ended; otherwise, they went to the robot-assignment step to start the next session.

After completing all the 15 sessions, the participants received a bonus determined by their average detection accuracy, which is designed to encourage them to gave their true trust feedback. The participants were told that giving true trust feedback would help the other participant to decide how much he or she would like to trust the drones and thus increase their detection accuracy. 

\subsection{Experiment Procedure}
A total of 22 participants (average age = 25.2 years, SD = 4.3 ages, 12 females, 10 males) with normal or corrected-to-normal vision participated in the experiment. Each participant received a \$15 base payment and an up-to \$10 bonus depending on their team performance. Prior to the experiment, each participant signed a consent form and filled out a demographic survey. Two practice sessions were provided to familiarize the participants with the detection tasks, where an AI acted as the assistant robot instead of the drones. The participants were told the reliability of the AI was different from the ones of the drones. The assignment of drones was randomized in each group. Specifically, we assigned drone $A$ with equal change to either the first or the second participant, and then assigned drone $B$ to the other participant. The reliabilities of the AI, drone $A$, and drone $B$ were set to 80\%, 90\%, and 60\%, respectively, across all the experiments.

\subsection{Data Analysis}
\input{fig_data_analysis}
We labeled the participant as $p_1,\dots,p_{22}$. First, we analyzed the average trust values on the robots at each session, namely, $\overline{t}_{A}( k) \equiv \sum _{i=1}^{22} t_{A}^{p_{i}}( k)$ and $\overline{t}_{B}( k) \equiv \sum _{i=1}^{22} t_{B}^{p_{i}}( k)$, $k=0,1,2,\dotsc ,15$, as shown in Fig.~\ref{fig:average_trust}. Average trust values on each robots stabilize after around first 5 sessions. The average initial trusts $\overline{t}_{A}( 0)$ and $\overline{t}_{B}( 0)$ are 0.56 and 0.60 with standard deviation 0.26 and 0.24. No significance was found on the difference of $t_A(0)$ and $t_B(0)$ ($p=0.11$, t-test). The average final trusts $\overline{t}_{A}(15)$ and $\overline{t}_{B}(15)$ are 0.82 and 0.48 with standard deviation 0.12 and 0.19. The final trust values $t_A(15)$ and $t_B(15)$ are significantly different($p<0.01$, t-test).

Second, we compared the difference of final trust values from participants in the same group and in different groups. A bar plot is shown in Fig.~\ref{fig:diff_final_trust}. The between-group final trust difference on $A$ and $B$ have mean values 0.12$\pm$0.11 and 0.21$\pm$0.16 and they are significantly different ($p<0.01$, t-test). The within-group final trust difference on $A$ and $B$ have mean values 0.07$\pm$0.09 and 0.06$\pm$0.09 and no significance was found on the difference ($p=0.79$, t-test ). The between-group difference on the final trust of $A$ is significantly greater than the within-group difference ($p=0.02$, Mann–Whitney U test), which is also true for robot $B$ ($p<0.01$, Mann–Whitney U test).

Third, we analyzed the average within-group trust difference across the sessions. For both drones, the within-group trust difference first decreased and then stabilized as the experiment went on, as shown in Fig.~\ref{fig:ave_diff_trust}. The final difference is significantly smaller for both drones under t-test (drone $A$: initial: 0.28$\pm$0.28, final: $0.07\pm$0.10, $p=0.03$; drone $B$: initial: 0.27$\pm$0.26, final: $0.06\pm$0.09, $p=0.03$).

\subsection{Model fitting}


\begin{figure*}[h]
  \centering
  \includegraphics[width=1\linewidth]{figs/fitting_30_grid_search.pdf}
  \caption{Fitting results. Red curves are for drone $A$ while blue curves are for drone $B$. The solid lines are the participants' trust feedback while the dashed lines are the expected trust value given by the model. The shaded areas indicate the 90\% probability interval of the Beta distribution at each session. The index $i$-$j$ stands for the $j$th participant in the $i$the group.}
  \label{fig:fitting_all}
\end{figure*}

\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{figs/para_hist.pdf}
  \caption{Histogram of model parameters. A value $\beta^{p_{17}}_B(0)=907$ is removed for plotting. $\beta^{p_{17}}_B(0)$ is large because the participant $p_{17}$ had very low trust on robot $B$. His trust history is shown in Fig.~\ref{fig:fitting_all} (9-1).}
  \label{fig:para_hist}
\end{figure}

\input{table_parameter}
\textcolor{red}{change the following part according to ....}
Each participant has six model parameters on each robot. For example, the parameter set, denoted as $\theta^x_A$, of participant $x$ on robot $A$ include $x$'s prior experiences $\alpha _{A}^{x}( 0)$ and $\beta _{A}^{x}( 0)$, the unit direct experience gains $s_{A}^{x}$ and $f_{A}^{x}$, and the unit indirect experience gains $\hat{s}_{A}^{x}$ and $\hat{f}_{A}^{x}$. Accordingly, we can compute the experience gains using Eq.~\eqref{eq:direct_update} and Eq.~\eqref{eq:indirect_update} and add them to the the initial experience $(\alpha^x_A(0), \beta^x_A(0))$ to get the experiences $(\alpha^x_A(k), \beta^x_A(k))$ at each session, $k=0,1,\dots,15$. We use maximum likelihood estimation (MLE) to find the optimal parameters, i.e.,
\begin{equation*}
\begin{aligned}
\theta _{A}^{x} = & \arg\max\log P\left(\text{data}\middle| \theta \right)\\
= & \arg\max\sum _{k=0}^{15}\log\operatorname{Beta}\left( t_{A}^{x}( k)\middle| \theta _{A}^{x}\right)\\
= & \arg\max\sum _{k=0}^{15}\log\operatorname{Beta}\left( t_{A}^{x}( k)\middle| \alpha _{A}^{x}( k) ,\beta _{A}^{x}( k)\right)\text{.}
\end{aligned}
\end{equation*}
The fitting results are shown in Fig.~\ref{fig:fitting_all}. A histogram of parameter values is shown in Fig.~\ref{fig:para_hist}. Tab.~\ref{tab:parameters} shows the mean and standard deviation of model parameters. We set the performance measurements of drone $A$ at session $k$ as $p_{A}( k) ={A( k)}/{10}$ and $\overline{p}_{A}( k) ={10-A( k)}/{10}$, where $A(k)$ is the number of correct choices $A$ made in session $k$; and we define $p_{B}( k)$ and $\overline{p}_{B}( k)$ similarly. To measure the performance of the model, we defined the expected trust value to be $$\overline{t}_{R}^{p_{i}}( k) =\alpha _{R}^{p_{i}}( k) /\left( \alpha _{R}^{p_{i}}( k) +\beta _{R}^{p_{i}}( k)\right), R\in\{A,B\},$$ the fitting error at each session for each participant as $$e_{R}^{p_{i}} (k)=\left| \overline{t}_{R}^{p_{i}} (k)-t_{R}^{p_{i}} (k)\right| ,\ R\in \{A,B\},$$ and computed the root mean squre error between the ground truth and the expected trust value given by



\begin{equation*}
\text{RMSE} =\left[\frac{1}{N}\sum _{R\in \{A,B\}}\sum _{k=0}^{15}\sum _{i=1}^{22}\left( e_{R}^{p_{i}} (k)\right)^{2}\right]^{1/2}
\end{equation*}

where $N=2\times 16 \times 22$ is the number of data points available. The result is $\text{RMSE}=0.093$.

For comparison, we considered a direct-update-only model, where only direct experience gains are added to the total experience. This model is equivalent to setting the unit indirect experience gains $\hat{s}^x_A$ and $\hat{f}^x_A$ as 0. We recalculated the model parameters under this setting and the corresponding error is $\text{RMSE}'=0.100$. A further comparison showed, for trust on drone $A$, there is no significance found on the difference between the fitting errors between the two models ($p=0.06$, t-test); however, for trust on drone $B$, the fitting error of the proposed model is significantly smaller that the one on the direct-update-only model ($p<0.01$, t-test).



\section{Discussion}\label{sec:discussion}
\subsection{Human-Subject Experiment}
We discuss several findings in the human-subject experiment. First, the significant difference of the final trust in drone $A$ and drone $B$ indicates that the drones' reliabilities affected the participants' trust, which agrees with the previous research~\cite{lee1992trust}. 

Second, the between-group final trust is significantly greater than the within-group final trust. This exhibits trust propagation did exist in the experiment. In our previous work~\cite{Guo2020_IJSR}, three patterns of trust dynamics were observed in the experiment, namely, Bayesian decision-maker, oscillator, and disbeliever, where the latter two are relatively rare in the data. However, in Fig.~\ref{fig:fitting_all}, we observe that two oscillators, 8-1 and 8-2, and two disbelievers, 9-1 and 9-2, appeared in pairs. This phenomenon indicates even rare trust behaviors can be transferred through trust propagation. 

Third, in Fig.~\ref{fig:ave_diff_trust}, we observe fluctuations around the 2nd and 3rd sessions. This is possibly due to the first switch of drones in the early sessions.

\subsection{Model Fitting}
In Fig.~\ref{fig:fitting_all}, the shaded regions indicate the 90\% confidence interval of the Beta distribution at each session. We observe that for some participants, such as 7-2 and 10-2, the proposed model can accurately fit the trust curve with a narrow confidence interval; while, for some participants, such as 5-2 and 8-1, the model cannot fit the trust curve due to trust oscillation. However, in the latter case, the fitted curve has a similar trend with the ground truth and can cover most data points with the 90\% confidence interval. 

Compared with the direct-update-only model, the proposed model has a smaller RMSE and, in terms of the fitting error, performed significantly better on drone $B$ while having a similar performance on drone $A$. This could be explained by the performance difference between the two drones. Because the number of correct choices each drone could make follows binomial distributions ($\operatorname{B}(10, 0.9)$ for $A$ and $\operatorname{B}(10, 0.6)$ for $B$), the variance of their performance are 0.09 and 0.24 respectively. The greater variance on drone $B$ may result in a need for more information to stabilize one's trust. As a result, the proposed model benefited from modeling the information-sharing mechanism in the team, i.e., trust propagation, and thus had a better performance on fitting drone $B$'s trust. However, as drone $A$'s performance was relatively consistent, the participants could stabilize their trust with less information, therefore the proposed model didn't benefit much from trust propagation.

\section{Conclusion} \label{sec:conclusion}
In this work, we proposed the TRUP framework to model trust propagation in a multi-agent human-robot team. An innovative indirect trust update model was developed to model trust propagation between humans. Analysis showed the model has desired asymptotic behavior under different types of repeated interactions. We conducted a human-subject experiment to examine trust dynamics in a multi-agent human-robot team. Results showed the difference of within-group trust was significantly smaller than the difference of between-group trust, implied trust propagation affected participants' trust. In addition, data showed rare trust dynamics of an agent, i.e., oscillators and disbelievers, could impact his or her teammate. We fitted the data with the proposed model. Results showed the proposed model could effectively capture the dynamics of trust with an RMSE of 0.093. Comparison with a direct-update-only model revealed that the TRUP framework benefited from the trust propagation mechanism and achieved better fitting performance on the low-reliable robot.

The results should be viewed in light of the following limitations: First, the robots' reliabilities were set fixed during the interaction. Further studies are needed to test whether the framework can fit trust for situations where the robots can learn over time. Second, we made two key assumptions on the model, i.e., human agents are cooperative and communicate trust as a one-dimensional number. Future research can consider different settings. For instance, if the human agents have different objectives, they may deceive each other by deliberately giving inaccurate trust feedback. In such a case, a richer form of trust representation can be utilized, e.g., adding an additional dimension for distrust. 
\input{2_Appendix}


==> fig_data_analysis.tex <==
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{figs/fig_average_trust.pdf}
%   \caption{Average trust on drone $A$ and drone $B$ across all participants index by session number. The shaded regions indicate the sample standard errors.}
%   \label{fig:average_trust}
% \end{figure}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{figs/fig_diff_final_trust.pdf}
%   \caption{Difference of final trust. }
%   \label{fig:diff_final_trust}
% \end{figure}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{figs/fig_average_diff_trust.pdf}
%   \caption{Average within-group trust difference. The shaded regions indicate the sample standard errors.}
%   \label{fig:ave_diff_trust}
% \end{figure}

\begin{figure}[!t]
  \centering
    \begin{subfigure}{1\columnwidth}
    \captionsetup{width=1\linewidth}
        \centering
        \includegraphics[width=1\columnwidth]{figs/fig_average_trust.pdf}
        \caption{Average trust on drone $A$ and drone $B$ across all participants indexed by session numbers. The shaded regions indicate the sample standard errors. \textcolor{blue}{Jessie: change the legend to within-team trust average in XX}}
        \label{fig:average_trust}
    \end{subfigure}

    \begin{subfigure}{1\columnwidth}
    \captionsetup{width=1\linewidth}
        \centering
        \vspace{10pt}
        \includegraphics[width=1\columnwidth]{figs/fig_average_diff_trust.pdf}
        \caption{Average within-group trust deviation. The shaded regions indicate the sample standard errors.\textcolor{blue}{Jessie: change the legend to within-team trust deviation in XX}}
        \label{fig:ave_diff_trust}
    \end{subfigure}
    
    \begin{subfigure}{1\columnwidth}
    \captionsetup{width=1\linewidth}
        \centering
        \vspace{5pt}
        % \includegraphics[width=1\columnwidth]{figs/fig_diff_final_trust.pdf}
        \includegraphics[width=1\columnwidth]{figs/fig_diff_initial_and_final_trust.pdf}
        \caption{Final trust deviation.}
        \label{fig:diff_final_trust}
    \end{subfigure}
    
    \caption{Data analysis.}
  \label{fig:data_analysis}
\end{figure}


==> table_parameter.tex <==
\begin{table}[b]
\caption{Values of model parameters}
% \caption*{\footnotesize In each cell, the values are ($\overline{J}_m \pm \text{std}(J_m), \overline{\hat{t}}_N \pm \text{std}(\hat{t}_N) $)}
\label{tab:parameters}
\centering
\scalebox{1}{
\begin{tabular}{c|c|c}
\hline
Parameter   & Drone $A$               & Drone $B$              \\ \hline
$\alpha(0)$ & 42.03 $\pm$ 63.37 & 30.79 $\pm$ 68.69 \\ \hline
$\beta(0)$  & 17.96  $\pm$ 25.27   & 25.28 $\pm$ 75.24    \\ \hline
$s$         & 64.56 $\pm$ 76.79  & 46.53 $\pm$ 103.59 \\ \hline
$f$         & 78.80 $\pm$ 99.84  & 83.89 $\pm$ 145.77 \\ \hline
$\hat{s}$   & 599.12 $\pm$ 1103.01  & 204.44 $\pm$ 520.84 \\ \hline
$\hat{f}$   & 170.97 $\pm$ 301.87  & 183.50 $\pm$ 374.86 \\ \hline
\end{tabular}

}
\vspace{-4mm}
\end{table}
